Theoretical Analysis of Learned Database Operations under Distribution Shift through Distribution Learnability

Use of machine learning to perform database operations, such as indexing, cardinality estimation, and sorting, is shown to provide substantial performance benefits. However, when datasets change and data distribution shifts, empirical results also show performance degradation for learned models, possibly to worse than non-learned alternatives. This, together with a lack of theoretical understanding of learned methods undermines their practical applicability, since there are no guarantees on how well the models will perform after deployment. In this paper, we present the first known theoretical characterization of the performance of learned models in dynamic datasets, for the aforementioned operations. Our results show novel theoretical characteristics achievable by learned models and provide bounds on the performance of the models that characterize their advantages over non-learned methods, showing why and when learned models can outperform the alternatives. Our analysis develops the distribution learnability framework and novel theoretical tools which build the foundation for the analysis of learned database operations in the future.

==> old_analysis_framework.tex <==
\if 0

\textbf{Analyzing Generalization Error}. Consider the model, $\hat{f}$, trained after $j$ using dataset $\mD^j$, then, after $k$ insertions, with $i=j+k$, we are interested in the \textit{generalization error} $\mathds{E}_{\mD\sim\chi}[\normx{\hat{f}-f_{\mD^i}}]$. We have that 
\begin{align}
    \label{eq:generalization_bound}&\overbrace{\mathds{E}_{\mD\sim\chi}[\normx{\hat{f}-f_{\mD^i}}]}^{\text{Generalization Error}}\leq\\
    \nonumber&\qquad\underbrace{\mathds{E}_{\mD\sim\chi}[\normx{\hat{f}-f_{\mD^j}}]}_{\text{Modeling Error} }+\underbrace{\mathds{E}_{\mD\sim\chi}[\normx{f_{\mD^j}-f_{\mD^i}}]}_{\text{Data Drift}}. 
\end{align}

That is, we can bound the generalization error use \textit{modeling error}, $\mathds{E}_{\mD\sim\chi}[\normx{\hat{f}-f_{\mD^j}}]$, which is the error of modeling a set of observations (i.e., $\hat{f}$ is trained using $\mD^j$) and data drift, $\mathds{E}_{\mD\sim\chi}[\normx{f_{\mD^j}-f_{\mD^i}}]$, which is the expected change in the operation outputs due to the change in the dataset. 

Note that Ineq~\ref{eq:generalization_bound} implies that low modeling error does not necessarily guarantee low generalization error. This is expected, as the error should depend on how the dataset changes after the model is trained. Data drift is a statistical phenomenon and can be analyzed independent of the modeling choice, as the next lemma shows.

\begin{lemma}\label{lemma:data_drift}
    Assume $D$ consists of $i$ i.i.d samples. For $f\in\{r, c\}$, we have that that $\mathds{E}_{\mD\sim\chi}[\normx{f_{\mD^j}-f_{\mD^i}}]\leq 2\sqrt{i-j}$. Furthermore, for large enough $i$, $\mathds{E}_{\mD\sim\chi}[\normx{f_{\mD^j}-f_{\mD^i}}]\geq C\sqrt{i-j}$. 
\end{lemma}

The lemma shows that data drift is expected to be proportional to the square root of number of insertions after the model was trained. This means that even if we train perfect models with zero modeling error, the generalization error will be at least $\sqrt{k}$ after $k$ insertions. Note that Lemma~\ref{lemma:data_drift} assumes there is no distribution shift, and that the difference between $f_{\mD^j}$ and $f_{\mD^i}$ is only due to the randomness in sampling. As such, the $\sqrt{k}$ is indeed a lower bound on data drift, since data drift will be more pronounced if the data distribution shifts, as discussed in Sec. XXX. 

Lemma~\ref{lemma:data_drift} has two important consequences that shape the rest of the discussion and design choices in this paper. 

\textit{Need for specialization}. To obtain constant error, using a single model to answer queries is unlikely to work. Unless the model is retrained every constant number of operations (which leads to significantly large insertion time) the error will have to depend on data size. To be able to guarantee any desired accuracy, we need to somehow partition the space so that not every insertion affects every model (OR SOME OTHER REASON WHY PARTIONING WORKS). 

\textit{Relaxed Modelling Error}. Modeling error is fine to within $\sqrt{k}$. 

\fi


\if 0
insertion so that $\normx{\hat{f}-f_{\mD^i}}\leq \epsilon_1$. We are interested in studying the model error after $k$ more insertions, i.e., to understand how well the model approximates the operation function $f_{\mD^{i+k}}$ on the dataset $\mD^{i+k}$. The error is $\normx{f_{\mD^{i+k}}-\hat{f}}$. We call $\normx{\hat{f}-f_{\mD^i}}$ \textit{modeling error}, and $\normx{f_{\mD^{i+k}}-\hat{f}}$ \textit{generalization error}. Modeling error refers to the error of a model on the dataset it was trained on. Generalization error is the error of the model on a new dataset which the model was not trained on and had not seen before. One expects the modeling error to depend on generalization error. However, low modeling error does not guarantee low generalization error, as the generalization error also depends on the difference between $f_{\mD^{i+k}}$ and $f_{\mD^{i+k}}$. 

To make things formal, the missing piece is to add randomness. As the data is sampled from a data distribution, we can only provide probabilistic guarantees based on the distribution the data was sampled from. That is we are interested in analyzing $\mathds{P}_{\mD\sim\chi}(\normx{f_{\mD^{i+k}}-\hat{f}}\geq \epsilon)$ and ensuring that this probability is low enough. Note that 

\begin{align*}
    &\overbrace{\mathds{P}_{\mD\sim\chi}(\normx{f_{\mD^{i+k}}-\hat{f}}\geq \epsilon)}^{\text{generalization error}}\leq \\
    &\underbrace{\mathds{P}_{\mD\sim\chi}(\normx{f_{\mD^{i}}-\hat{f}}\geq \frac{\epsilon}{2})}_{\text{modeling error}}+\underbrace{\mathds{P}_{\mD\sim\chi}(\normx{f_{\mD^{i+k}}-f_{\mD^{i}}}\geq \frac{\epsilon}{2})}_{\text{distribution shift}}
\end{align*}

As such, we can analyze the generalization error in terms of modeling error and distribution shift. The distribution shift term above is used to quantify how the answers change as new data is inserted. We next discuss how each we analyze each term. 

PROPOSITION THAT EXPECTED VALUE OF THE SECOND TERM IS MAX $\sqrt{k}, \delta k$
\fi



\subsection{Distribution Model Oracle}
We use an oracle to abstract away the modeling problem and focus on how the models can be used to answer queries. We assume that we have access to an oracle that can create a model with bounded modeling error as in Ineq XXX, so that we can focus on how such a model can be used to provide desired final error guarantees. That is, this helps us study how to use learned models so that guarantees on the accuracy of models translate to the accuracy of performing a downstream task. 

To that end, we present the Distribution Model Oracle (DMO), that is an oracle that, given a set of observations, will return an accurate model of data distribution with high probability, specifically 



\begin{definition}
    A Distribution Model Oracle (DMO) for modeling a function $f_\chi$ for data distribution, $\chi\in\mathfrak{X}$, from a distribution class $\mathfrak{X}$ is an oracle that takes a set of observations, $\mD$, of size $n$ as input and returns a model $\hat{f}$ such that 
    \begin{itemize}
        \item If $\mD$ is sampled from $\chi$, for some  $\chi\in\mathfrak{X}$, we have that $\mathds{P}_{D\sim\chi}[\normx{f_\chi-\hat{f}}_\infty\geq \sqrt{n}\epsilon]\leq 2e^{-2\epsilon^2}$ for $\epsilon \geq 0$,
        \item It takes $\mathcal{T}_n^{\mathfrak{X}}$ number of operations to evaluate $\hat{f}$ and  space $\mathcal{S}_n^{\mathfrak{X}}$ to store it; and 
        \item Each call to the oracle costs $\mathcal{B}_n^{\mathfrak{X}}$.
    \end{itemize}
\end{definition}

IF $f_\chi$ is c.d.f OR ALMOST c.d.f WE CALL IT A c.d.f DMO
$f_\chi$ only depends on the data distribution, and the distribution model oracle returns a function, based on the observed data, that models this distribution dependent function \textit{well}, with high probability. We call $\hat{f}$ a \textit{distribution model}. XXX

DISCUSS POSSIBLE FUNCIONS, GIVE EXAMPLES, ...

Note that $\mathcal{T}_n$, $\mathcal{S}_n$ and $\mathcal{B}_n$ are properties of the oracle. XXXDISCUSS Furthermore, if the observations were sampled from a distribution, $\chi$, with c.d.f $F_\chi$, . 
    

The problem of modeling the data distribution is a typical function approximation/statistical learning problem, where the goal is to model the data distribution given a set of observations. Different modeling choices are possible depending on the assumption on the data distribution. 

We present the following lemmas to show that such oracles exist, GENERALIZATION OF X, even under mild assumptions on data distribution 
E.g., we have 

\begin{lemma}
    Assume a dataset $\mD$ consists of $n$ points such that $D_i$ is sampled independently, from some distribution $\chi_i$. Assume that, for all $i$, the p.d.f of $\chi_i$ is bounded by $\rho$, all distributions are defined over the domain $[a, b]$. Let $\mathfrak{X}$ be all possible data distributions defined by the above sampling procedure.   
    Let $F_\chi=\frac{1}{n}\sum_{i=1}^nF_{\chi_{i}}$, where $F_{\chi_{i}}$ is the c.d.f of $\chi_i$. There exists a DMO for $F_\chi$, $\chi\in\mathfrak{X}$  with parameters $\mathcal{B}_n=O((b-a)\rho\sqrt{n})$, $\mathcal{T}_n=O(1)$ and $\mathcal{S}_n=O((b-a)\rho\sqrt{n})$. 
\end{lemma}

%such that $\mathds{P}(\normx{kf_{\chi}^{i, j}-\hat{f}}_\infty\geq \sqrt{k}(2\epsilon+1))\leq 4e^{-2\epsilon^2}$ for $\epsilon\geq 0$, and

\subsection{Analyzing Conditional Distribution Models}
We will not only model the entire distribution but model conditional parts of it. 


\textbf{Modeling Conditional Distribution}. When using models to answer queries, we often partition the space and build models specialized for certain parts of the space. Such models can be seen as models of the conditional probability distribution, conditioned that the points sampled from the distribution fall in the region of the space modeled. We say a distribution class, $\mathfrak{X}$ over a domain $\mathcal{D}$ is \textit{closed under conditioning} (or CC for short) w.r.t a set $\mathcal{R}\subset2^{\mathcal{D}}$ if for any $R\in\mathcal{R}$ and for all $\chi\in\mathfrak{X}$, $\chi|R$ is also in $\mathfrak{X}$. In this paper, unless otherwise stated, $\mathcal{R}$ is the set of axis-parallel rectangles. This is because the partitioning methods we consider only partition the space using axis-parallel rectangles. As a result, we only need to consider data distribution conditioned over data falling in an access parallel rectangle. 

Note that conditioning only shifts, scales, and \textit{crops} the c.d.f. of the data distribution. Thus, if a class of distributions is invariant to scaling, it will be closed under conditioning. For instance, the uniform distribution is closed under conditioning. We can create a distribution closed under conditioning by simply adding all the conditioned distribution to the class. SHOW LEMMA FOR THE LAST STATEMENT. DOUBLE CONDITIONING DOESNT CAUSE PROBLEMS.  

\begin{lemma}
    Assume $\mathfrak{X}$ is the set of distributions with bounded and non-zero p.d.fs. That is, for any $\chi\in\mathfrak{X}$, $\exists \chi_{\rho_1}, \chi_{\rho_2}$ such that $0<\chi_{\rho_{1}}\leq f_\chi(x)\leq \chi_{\rho_{2}}<\infty$ for all $x$. $\mathfrak{X}$ is closed under conditioning. 
\end{lemma}

Means we can use Lemma XX not only on the distribution data is sampled from



\if 0
\begin{lemma}
    Assume $\rho_1$ is the maximum pdf value and $\rho_2$ is the minimum p.d.f value across $n$ distributions $\chi_1, ..., \chi_n$. Let $f_\chi^{i, j}=\frac{1}{k}\sum_{t=1}^kf_{\chi_{z_t}}$, where $f_{\chi_{z_t}}$ is the c.d.f of $z_t$-th element in the sorted subarray $A[i:j]$ and $k=j-i$. We can build a piecewise constant approximation, $\hat{f}$ of $f_\chi^{i, j}$ with $\frac{\rho_1}{\rho_2}\sqrt{k}$ pieces so that $\mathds{P}(\normx{kf_{\chi}^{i, j}-\hat{f}}_\infty\geq \sqrt{k}(2\epsilon+1))\leq 4e^{-2\epsilon^2}$ for $\epsilon\geq 0$. Given that the array is sorted and indexed, we have that $B(k)=O(\frac{\rho_1}{\rho_2}\sqrt{k})$, $T(k)=O(1)$ and $S(k)=O(\frac{\rho_1}{\rho_2}\sqrt{k})$. INCREMENTAL UPDATES?!
\end{lemma}

Assuming the data is independent samples, the best $\epsilon$ that can be achieved with high probability is $\frac{1}{\sqrt{n}}$ DUE TO EXISTING RESUTSL. SO OFTEN IT IS REDUNDANT TO BE MORE ACCURATE. Thus, we use $T_{n}=T_{n, \sqrt
{n}}$ for simplicity of notation, denoting when we approximate the distribution to $\frac{1}{\sqrt{n}}$ accuracy. 


First, we note that, in their generality, it is not necessarily true that there exist distribution models, with the desired accuracy requirements, and not all possible space/time trade-offs are known. Furthermore, it is also not true that, even if a model of a distribution exists, it can be found to any desired accuracy by only looking at $n$ samples from the distributions. Indeed, the number of samples required to learn a distribution has been a subject of study in statistical learning XXXX, furthermore, relationship between time complexity, space complexity and accuracy of models has been studied in function 
approximation XXX> 

\fi



\textbf{Quantifying Conditional Distribution Shift}
DMO uses observations up to a certain point to build a model of the data distribution. However, how well this model of data distribution generalizes to future observations depends on how the data distribution changes over time. 

We use two notions of distribution shift. First, we utilize the variational distance, which is the maximum different in probability of an event. Indeed, variational distance is a suitable notion to capture distribution shift in our problem. For example, in th case of cardinality estimation, for a query $q$, the expected query answer is $n\times \mathds{P}_{p\sim\chi}(p\in q)$. Therefore, if the data is sampled from another distribution $\chi$, the expected difference between the query answers is bounded by $n\delta$.  MAYBE SAY THIS AS A LEMMA

Thus, if we use a data distribution to answer queries, but data distribution shifts, we expect error liner in data size and distribution shift. This helps us characterize how often we need to retrain models. 

However, a bound on total variation is often not sufficient. This is because learned models are often used to model conditional distributions. This happens when models partition the space, where each model is responsible for answering queries for a specific part of the subspace. Such models can be seen as modeling the conditional data distribution, where the distribution is conditioned on data points falling into the modeled range. 

Here, we propose the notion of \textit{conditional total variation}, an extension of total variation , to quantify the distribution shift.  MAYBE SHOW THAT THE MAXIMUM IS NOT ACHIEVED IN THE LIMIT?

\begin{definition}
    Given two probability distributions $\chi_1$ and $\chi_2$ defined over $(\Omega, \mathcal{F})$, the conditional total variation is defined as $\sup_{A\in \mathcal{F}, \chi_1(A),\chi_2(A)\neq 0}\sup_{B\in \mathcal{F}}|\frac{\chi_1(B\cap A)}{\chi_1(A)}-\frac{\chi_2(B\cap A)}{\chi_2(A)}|$  
\end{definition}

NOT SURE IF THIS IS WELL DEFINED, WRITE THIS USING MORE BASIC PROBABILITY NOTATION AND PERHAPS LESS GENERAL CONDITIONING, JUST AS MUCH AS YOU NEED.

NEED TO SHOW THIS IS WELL DEFINED AND NOT STUPID

\subsection{The Distribution Oracle Analysis Framework}

DISCUSS HOW THE RESULTS WILL LOOK LIKE

==> old_oracle_construction.tex <==

\subsection{Constructing Oracles}
%We need to show the existence of different oracles
In this section, we show how we can create oracles for different distribution classes. We first show that the problem of constructing oracles can be seen purely from a function approximation perspective, abstracted away from the application of learning database operations. Using this result, we then show how to construct oracles for distributions with bounded p.d.f or piece-wise linear c.d.f. We note that abstracting the problem of oracle construction as a generic function approximation problem has far-reaching consequences because this, combined with our results in Sec.~\ref{sec:using_oracles}, means our framework allows us to translate generic function approximation results to provide methods that perform learned database operations under distribution shift with theoretical guarantees. Thus, as more becomes known about the function approximation ability of a certain function class (e.g., neural networks) in the future, our framework immediately translates such results to bounds on performing learned database operations. 


%Informally, we first show that if a function class $\mathcal{F_1}$ can be used to approximate another function class $\mathcal{F}_2$ \textit{well}, then we can use $\mathcal{F_1}$ to construct an oracle for distributions with c.d.f in $\mathcal{F}_2$. %Given that c.d.f of a distribution can be any right-continuous non-decreasing function that increases from 0 to 1, any function approximation result where the set $\mathcal{F}_2$ contains functions with these properties can be applied to obtain oracles for the corresponding distribution classes. 
%Moreover, our results in Sec.X show how an oracle can be used to perform database queries. Thus, combining these two results means our framework allows us to translate generic function approximation results to provide methods that perform learned database operations with theoretical guarantees. 


%We present a generic way of creating oracles using existing function approximation results. 
Informally, we first show that if a function class $\mathcal{F_1}$ can be used to approximate another function class $\mathcal{F}_2$ \textit{well}, then we can use $\mathcal{F_1}$ to construct an oracle for distributions with c.d.f in $\mathcal{F}_2$. Indeed, different function approximation classes are suitable for different distribution classes. For instance, a linear model may be sufficient to approximate data from a uniform distribution, while a Gaussian model may be more suitable for bell-shaped distributions. %In fact, if our goal is to model the c.d.f of the data distribution, then we should ensure that the function class can effectively model the c.d.f. 
%Meanwhile, given that we care about the efficiency of the function approximation as well as its accuracy, we want to ensure that we achieve a desired level of accuracy with the most efficient model possible within the function class.

We first present definitions, helping us quantify what it means to approximate a function class well. Consider using $\mathcal{F}$ (e.g., piecewise constant fucntions) to approximate a function $f$. There is often a trade-off between the efficiency and accuracy of the approximator (e.g., a piece-wise constant function with more pieces is less efficient but more accurate). Thus, given an accuracy requirement, we allow restricting the class of functions used for approximation to the ones that achieve the desired accuracy but are suitably efficient. For instance, we may bound the number of pieces to $t_\epsilon$ when using piece-wise constant function approximations to achieve accuracy $\epsilon$. Thus, from our original function class $\mathcal{F}$, we may only use the subset $\mathcal{F}_\epsilon$ when we want to approximate a function to accuracy $\epsilon$. Moreover, the relationship between $\epsilon$ and $t_\epsilon$ should depend on $f$, because if $f$ is difficult to approximate, we should use more pieces even if $\epsilon$ is large. This notion of what subset of the original function approximation class to use when approximating another function class to a desired accuray is formalized by defining \textit{approximation system} below. 

\begin{definition}
A \textit{function approximation system}, for a function class $\mathcal{F}$ approximating a distribution class $\mathfrak{X}$ is a nested set of subsets of $\mathcal{F}$, $\mathcal{F}_\epsilon\subseteq \mathcal{F}$, with $\mathcal{F}_\epsilon\subseteq \mathcal{F}_{\epsilon'}$ whenever $\epsilon\leq \epsilon'$, where for any $\chi\in\mathfrak{X}$ and $\epsilon>0$, there exists a function, $\hat{f}_\chi\in \mathcal{F}_\epsilon$ for which $\normx{\hat{f}_\chi-f_\chi}_\infty\leq \epsilon$. 
\end{definition}

\begin{definition}
An \textit{approximation system}, for a function class $\mathcal{F}$ approximating another function class $\mathcal{F}'$ is a nested set of subsets of $\mathcal{F}$, $\mathcal{F}_\epsilon\subseteq \mathcal{F}$, with $\mathcal{F}_\epsilon\subseteq \mathcal{F}_{\epsilon'}$ whenever $\epsilon\leq \epsilon'$, where for any $f\in\mathcal{F}'$ and $\epsilon>0$, there exists a function, $\hat{f}\in \mathcal{F}_\epsilon$ for which $\normx{\hat{f}-f}_\infty\leq \epsilon$. 
\end{definition}


The following proposition provides an example for a function approximation system, showing that we can build a function approximation system using the class of piecewise constant functions, $\mathcal{P}$, for the class of distributions with bounded derivative. 

\begin{proposition}
    Let $\mathfrak{X}_\rho$ be the class of data distributions over $[0, 1]$ with their p.d.f bounded by $\rho$, and let $\mathcal{P}_\epsilon$ be the subset of $\mathcal{P}$ with at most $\frac{\rho}{\epsilon}$ pieces. For any $\chi\in \mathfrak{X}_\rho$ and any $\epsilon>0$, there exists $\hat{f}_\chi\in\mathfrak{P}_\epsilon$ s.t. $\normx{\hat{f}_\chi-f_\chi}_\infty\leq \epsilon$. Thus, $\{\mathcal{P}_\epsilon, \epsilon>0\}$ is a function approximation system for $\mathfrak{X}_\rho$. 
\end{proposition}

\begin{proposition}
    Let $\mathcal{F}'$ be the class of real-valued functions over $[0, 1]$ with their derivative bounded by $\rho$, and let $\mathcal{P}_\epsilon$ be the subset of $\mathcal{P}$ with at most $\frac{\rho}{\epsilon}$ pieces. For any $f\in \mathcal{F}'$ and any $\epsilon>0$, there exists $\hat{p}\in\mathfrak{P}_\epsilon$ s.t. $\normx{\hat{p}-f}_\infty\leq \epsilon$. Thus, $\{\mathcal{P}_\epsilon, \epsilon>0\}$ is a function approximation system for $\mathcal{X}$. 
\end{proposition}

In plain terms, we can approximate a function with derivate $\rho$ with at most $\frac{\epsilon}{\rho}$ number of pieces. Thus, if our data distribution has c.d.f at most $\rho$, we can approximate it with a member of $\mathcal{P}_\epsilon$ and have error at most $\epsilon$. As a result, not only we know that we can approximate the c.d.f with $\mathcal{P}$ with any desired accuracy, but we also know that to obtain error $\epsilon$ $\frac{\rho}{\epsilon}$ number of pieces is sufficient. Thus, having a function approximation system allows us to only use as much model capacity as needed, therefore allowing us to bound the inference complexity. 


Nonetheless, having just a function approximation system is not sufficient to have an oracle for a distribution class. This is because, even if a function approximating the c.d.f exists in the function class, there is no guarantee we can find it. Thus, it is additionally required that we can find the best approximator within the class (best is actually not required, but we don't generalize here), which is formalized next.

\begin{definition}
    A function approximation system is \textit{optimally solvable} if there exists an algorithm $\mathfrak{A}$ that, given any parameter $\epsilon>0$ and any function $f$ can find the $\infty$-norm best approximation to $f$ in $\mathcal{F}_\epsilon$. That is, $\mathfrak{A}(f, \epsilon)=\arg\min_{f'\in\mathcal{F}}\normx{f-f'}_\infty.$
\end{definition}

%That is, we should be able to find $\arg\min_{f'\in\mathcal{F_\epsilon}}\normx{f-f'}_\infty$, for functions $f$. We call a function approximation system optimally solvable if 
%The following lemma shows that if the two conditions are satisfied, we can construct an oracle. 
The following lemma shows that an optimally solvable function approximation system an be used to build a distribution model oracle. 


\if 0
A function approximation system helps formalize the intuitions mentioned above. For example, assume $\mathcal{F}$ is the set of piecewise constant functions. We set that $\mathcal{F}_\epsilon$ is the set of piecewise constant functions with at most $\frac{1}{\epsilon}$ pieces. 

. In other words, depending on the assumptions made on the data distribution, different model classes may be suitable for modeling the data distribution. 


. Informally, our result states that if for a function $f$, we can find the optimal function approximator from some function class $\mathcal{F}$, and that for some distribution class $\mathfrak{X}$, the function class $\mathcal{F}$ is a good approximator o

\fi
% (i.e., $\mathfrak{A}$ can evaluate $f(x)$ for any $x$)
\begin{theorem}    
    Assume we have an optimally solvable function approximation system, $\mathfrak{F}$ for a function class $\mathcal{F}'$, with the optimizor $\mathfrak{A}$, and let $\mathfrak{X}$ be a class of distributions s.t. $f_\chi\in \mathcal{F}'$.
    Then, for a dataset of size $n$, algorithm $\mathfrak{A}(., \frac{1}{\sqrt{n}})$ is a distribution model oracle for the distribution group $\mathfrak{X}$, with $\mathcal{T}_n^\mathfrak{X}$ and $\mathcal{S}_n^\mathfrak{X}$ the maximum time and space complexity of any function in $\mathcal{F}_{\frac{1}{\sqrt{n}}}$, and $\mathcal{B}_n^\mathfrak{X}$ the number of operations to call $\mathfrak{A}$.
\end{theorem}


\begin{theorem}    
    Assume we have an optimally solvable function approximation system, $\mathfrak{F}$ for a distribution class $\mathfrak{X}$, with the optimizor $\mathfrak{A}$. % that, given any parameter $\epsilon>0$ and any function $f$ can find the $\infty$-norm best approximation to $f$ in $\mathcal{F}_\epsilon$. That is $$\mathfrak{A}(f, \epsilon)=\arg\min_{f'\in\mathcal{F}}\normx{f-f'}_\infty.$$
    %and a set of function classes $\mathcal{F}=\{\mathcal{F}_\epsilon, \forall\epsilon>0\}$ , where $\mathcal{F}_{\epsilon_1}\subseteq \mathcal{F}_{\epsilon_2}$ for all $\epsilon_1\leq \epsilon_2$ returns a function $f^*\in \mathcal{F}_\epsilon$ s.t. $\normx{f-f^*}_\infty\leq \normx{f'-f}_\infty$ for all $f'\in \mathcal{F}_\epsilon$. 
    Then, for a dataset of size $n$, algorithm $\mathfrak{A}(., \frac{1}{\sqrt{n}})$ is a distribution model oracle for the distribution group $\mathfrak{X}$, with $\mathcal{T}_n^\mathfrak{X}$ and $\mathcal{S}_n^\mathfrak{X}$ the maximum time and space complexity of any function in $\mathcal{F}_{\frac{1}{\sqrt{n}}}$, and $\mathcal{B}_n^\mathfrak{X}$ the number of operations to call $\mathfrak{A}$.
\end{theorem}

Thus, if we show we can find the best approximator in the class of piecewise constant functions, we can show there exists an oracle for the class of distributions with bouded p.d.f. This is shown in the next lemma, together with more results showing existence of oracles for other distribution classes. 

\begin{lemma}
    For any function $f$ and any $\epsilon>0$, there exists an algorithm, $\mathfrak{P}$, that finds the best $\infty$-norm approximation to $f$ in $\mathcal{P}_\epsilon$. Therefore, There exists a distribution model oracle for $\mathfrak{X}_\rho$.
\end{lemma}

\if 0
\begin{lemma}
    Let $\mathfrak{X}_\rho$ be the class of data distributions over $[0, 1]$ with their p.d.f bounded by $\rho$. For any $\chi\in \mathfrak{X}_\rho$ and any $\epsilon>0$, there exists $\hat{f}_\chi\in\mathfrak{P}_\epsilon$ s.t. $\normx{\hat{f}_\chi-f_\chi}_\infty\leq \epsilon$.
\end{lemma}

\begin{corollary}
    
\end{corollary}
\fi


\if 0
\begin{lemma}
    Let $\mathfrak{X}_{\rho, \rho'}$ be the set of data distributions with p.d.f between $0<\rho\leq f_\chi(x)\leq \rho_2<\infty$. The set $\mathfrak{X}_{\rho, \rho'}$ is closed under conditioning. XXX
\end{lemma}


We present the following lemmas to show that such oracles exist, GENERALIZATION OF X, even under mild assumptions on data distribution 
E.g., we have 

\begin{lemma}\label{lemma:piecewise_constant_oracle}
    Assume a dataset $\mD$ consists of $n$ points such that $D_i$ is sampled independently, from some distribution $\chi_i$. Assume that, for all $i$, the p.d.f of $\chi_i$ is bounded by $\rho$, all distributions are defined over the domain $[a, b]$. Let $\mathfrak{X}$ be all possible data distributions defined by the above sampling procedure.   
    Let $F_\chi=\frac{1}{n}\sum_{i=1}^nF_{\chi_{i}}$, where $F_{\chi_{i}}$ is the c.d.f of $\chi_i$. There exists a DMO for $F_\chi$, $\chi\in\mathfrak{X}$  with parameters $\mathcal{B}_n=O((b-a)\rho\sqrt{n})$, $\mathcal{T}_n=O(1)$ and $\mathcal{S}_n=O((b-a)\rho\sqrt{n})$. 
\end{lemma}




\begin{lemma}\label{lemma:piecewise_constant_cc}
    Assume $\mathfrak{X}$ is the set of distributions with bounded and non-zero p.d.fs. That is, for any $\chi\in\mathfrak{X}$, $\exists \chi_{\rho_1}, \chi_{\rho_2}$ such that $0<\chi_{\rho_{1}}\leq f_\chi(x)\leq \chi_{\rho_{2}}<\infty$ for all $x$. $\mathfrak{X}$ is closed under conditioning. 
\end{lemma}

Means we can use Lemma XX not only on the distribution data is sampled from

\fi



PROOFS 



\subsection{General X}


Recall that an oracle takes a dataset, $\mD$, of size $n$, as an input. Given such a dateset, we return  $\hat{f}=\frac{1}{n}\mathfrak{A}(f_{\mD}, \frac{1}{\sqrt{n}})$ for $f\in \{r, c\}$ as our model of $f_\chi$. To analyze the accuracy of such a model, observe that, for any input $x$ we have
\begin{align*}
    |\hat{f}(x)-\frac{1}{n}f_{\mD}(x)|&\leq |\hat{f}_\chi(x)-\frac{1}{n}f_{\mD}(x)| \\
    &\leq |\hat{f}_\chi(x)-f_\chi(x)|+|f_\chi(x)-\frac{1}{n}f_{\mD}(x)|\\
    &\leq \frac{1}{\sqrt{n}}+|f_\chi(x)-\frac{1}{n}f_{\mD}(x)|.
\end{align*}
We also have $|\hat{f}(x)-f_\chi(x)|\leq |\hat{f}(x)-\frac{1}{n}f_{\mD}(x)|+|f_\chi(x)-\frac{1}{n}f_{\mD}(x)|$, so that 
$$
|\hat{f}(x)-f_\chi(x)|\leq \epsilon+2|f_\chi(x)-\frac{1}{n}f_{\mD}(x)|
$$
By Hoeffeding's inequality, we have
\begin{align}
    \mathds{P}(|nf_\chi(x)-f_{\mD}(x)|\geq \epsilon')\leq e^{-2(\frac{\epsilon'}{\sqrt{n}})^2},
\end{align}
So that 
\begin{align}
    \mathds{P}(n|f_\chi(x)-\hat{f}(x)|\geq 2\epsilon'+n\frac{1}{\sqrt{n}})\leq e^{-2(\frac{\epsilon'}{\sqrt{n}})^2},
\end{align}
And therefore, 
 \begin{align}
    \mathds{P}(n|f_\chi(x)-\hat{f}(x)|\geq \epsilon)\leq e^{-\frac{1}{2}(\frac{\epsilon}{\sqrt{n}}-1)^2}.
\end{align}


%Furthermore, assume the function $\f_\chi\in \mathcal{F}$ and that $|f-f_\chi|\leq \epsilon$. Therefore, for $f^*=A(f)$, we have $|f-f^*|\leq |f-f_\chi|+|\hat{f}\epsilon+||$

\subsection{Proof of Lemma~\ref{lemma:piecewise_constant_oracle}}

Let $\mathfrak{X}$ be the set of distributions with p.d.f bounded by $\rho$. %bounded p.d.f, that is, for any $\chi\in\mathfrak{X}$ we have $f_\chi(x)\leq \rho_\chi$, for $\rho_\chi<\infty$. 
Let $\mathcal{F}$ be the set of piecewise constant functions, and let $\mathcal{F}_\epsilon$ be the set of piecewise constant functions with at most $\frac{\rho}{\epsilon}$ pieces. 


First, note that the error of approximation goes down as the number of pieces increases, that is, the best approximation with $i$ pieces is at least as good as the best approximation with $j$ pieces, $j<i$. Thus, we consider building the best approximation with $\frac{\rho}{\epsilon}$ pieces. To minimize the infinity norm error, we place a constant at the mid-point of max and minium value in each interval.  This shows that we can solve the problem optimally. 

Next, we show that for any $\chi\in \mathfrak{X}$ and any $\epsilon>0$, there is a function $\hat{f}_\chi\in \mathcal{F}_\epsilon$ s.t. $\normx{\hat{f}_\chi-f_\chi}_\infty\leq \epsilon$. This function is the optimal solution as constructed above. To see why the error is at most $\epsilon$, consider the $i$-th partition over $I=[p_i, p_{i+1}]$, where $p_{i+1}-p_i=\frac{\epsilon}{\rho}$, and let $x_1$ and $x_2$ be the two points in $I$ that, respectively, achieve the minimum and maximum of $f_\chi$ in $I$. For any point in $x\in I$, our function approximator answer $\hat{f}(x)=\frac{1}{2}(f_{\chi}(x_1)+f_{\chi}(x_2))$. We have that 
\begin{align*}
    |\hat{f}(x)-f_\chi(x)|&=|\frac{1}{2}(f_{\chi}(x_1)+f_{\chi}(x_2))-f_\chi(x)|\\
    &\leq \max\{f_{\chi}(x_2)-f_\chi(x), f_\chi(x)-f_{\chi}(x_1)\}\\
    &\leq |f'_\chi(x)(x_2-x)|\\
    &\leq \rho\frac{\epsilon}{\rho}=\epsilon.
\end{align*}

%Let for any $\chi$, with maximum p.d.f. $\rho_\chi$, a piecewise constant function, $\hat{f}_\chi$ with $\frac{\rho_\chi}{\epsilon}$ pieces s.t. $\normx{\hat{f}_\chi-f_\chi}_\infty\leq \epsilon$


\subsection{Proof of~\ref{lemma:piecewise_constant_cc}}




==> old_proof_dyn_indx_rebuild_logarithmic_all.tex <==
\if 0
\begin{algorithm}[t]
\begin{algorithmic}[1]
\Require New element to be inserted in tree rooted at $N$
\Ensure Balanced data structure
\Procedure{Insert}{$p$, $N$}
    \If{$N.children==\text{NULL}$}
        \State $N.content.insert\_sorted(p)$
        \State $N.counter++$
        \State \Return
    \EndIf
    \State $\hat{i}\leftarrow N.\hat{f}(p)$
    \State $i\leftarrow ExpSearch(p, \hat{i}, N.content)$
    \State Insert($P$, $N.children[i]$)
    \State $N.counter++$
    \If{$N.counter==N.max\_points$}
        \State $A\leftarrow$ sorted array for subtree rooted at $N$
        \State $N\leftarrow$ Rebuild($A$)
    \EndIf 
\EndProcedure
\Require New element to be inserted in tree rooted at $N$
\Ensure Balanced data structure
\Procedure{Rebuild}{$A$}
    \State $N\leftarrow$ new node
    \State $k\leftarrow |A|$
    \If{$k\leq c$}
        \State $N.content=A$
        \State \Return $N$
    \EndIf    
    \State $N.max\_points=2k$
    \State $N.\hat{f}=\textsc{BUILD}(A, k, \sqrt{k})$
    \State $N.content=A[::\sqrt{k}]$
    \For{$i$ in $\sqrt{k}$}
        \State $N.children.append(Rebuild(A[i k:(i+1)k]))$
    \EndFor
\EndProcedure

\caption{Dynamic Learned Index}\label{alg:dynamic_learned_index}
\end{algorithmic}
\end{algorithm}


\subsection{Proof of Theorem \ref{thm:dynamic_indexing_oracle}}

We assume, for every subset of $A$, of size $k$, there exists a distribution model with error $\frac{1}{\sqrt{k}}$ that can built in $B_k$ operations, can be evaluated in $T_k$ operations and takes space $S_k$ bits. 

\textbf{Index  Construction}. The index construction is presented in Alg. X. The index is a tree, where each node is associated with a model, content and size limit. Size limit of a node is the maximum allowed number of total points in the subarray indexed by the tree rooted at the node. If a node is a leaf but not a root, there is no maximum. If the node is a leaf, it's content are the data to be indexed. If it's a non-leaf node, the content are used to index it's children, as in a typical B-tree. However, the content is always searched by the model of the node, (and not by binary search, as done in a B-tree). If a node becomes full, the entire sub-tree rooted at the node is rebuilt. At rebuilding, the capacity of a non-leaf node is set to double its current size. A node is built to have children if its size is at least $C$, for some constant integer $C$ that is a system parameter.

\textbf{Query}. 


\textbf{Insertion Time Analysis}.  It's log n amoretized in case there is distribution shift, but without/with less distribution shift, it should be loglog n. NEITHER ARE FULLY PROVEN HERE


First, assume after $k$ insertions the root has been rebuilt, and consider the next $k$ insertions until the root is rebuilt again.

First, we show that the content of each non-leaf node can be searched in expected constant time using the model associated with each node. Note that neither the content of each node, nor its model gets modified by insertions, unless a node is rebuilt. Thus, we only need to show the statement for right after the node construction. Assume the node is constructed for some array $A$ with $|A|=l$ for some integer $l$, and thus, the content of the node is $A[::\sqrt{l}]$. Now recall that elements of $A$, $A[1]$, ..., $A[l]$ are independent samples some distributions $\chi_1$, ..., $\chi_n$ respectively THE ACUTAL DISTRIBUTION IS CONDITIONED ON THE RANGE XXX. By the extended DKW bound, we have that 

$$
\mathds{P}(\normx{f_\chi-f_n}_\infty\geq \epsilon)\leq 2e^{-2n\epsilon^2}
$$

Furthermore, for our model of $\frac{1}{l}\sum_{i=1}^lf_{\chi_l}$, $\hat{f}$, we also have that  

$$
\mathds{P}(\normx{f_\chi-\hat{f}}_\infty\geq \epsilon)\leq 2e^{-2n\epsilon^2}
$$

So that, by union bound

$$
\mathds{P}(\normx{f_\chi-\hat{f}}_\infty\geq \epsilon \text{ or } \normx{f_\chi-f_n}_\infty\geq \epsilon)\leq 4e^{-2n\epsilon^2}
$$

and that 
$$
\mathds{P}(\normx{f_\chi-\hat{f}}_\infty\leq \epsilon \text{ and } \normx{f_\chi-f_n}_\infty\leq \epsilon)\geq 1-4e^{-2n\epsilon^2}
$$

and therefore

$$
\mathds{P}(\normx{f_n-\hat{f}}_\infty\leq \epsilon)\geq 1-4e^{-\frac{1}{2}n\epsilon^2}
$$

Now recall that we use $\ceilx{\sqrt{l}\hat{f}(x)}$ as an estimate for the location in content to search for $x$. For the estimated location $\hat{i}$ and true location $i$, we have that $|i-\hat{i}|=t$ implies that $l\normx{f_n-\hat{f}}_\infty\geq (t-2)\sqrt{l}$. Furthermore, note that if the exponential search takes $N$ operations, starting from $\hat{i}$ to find $i$, the then $t\geq 2^\frac{N-1}{2}$. Using these we have that the 

\begin{align*}
    \mathds{E}_{A\sim\chi}[N] &= \sum_{i=1}^{2\log l}\mathds{P}_{A\sim\chi}(N\geq i)\\
    &\leq  \sum_{i=1}^{2\log l}\mathds{P}_{A\sim\chi}(t\geq 2^\frac{i-1}{2})\\
    &\leq  \sum_{i=1}^{2\log l}\mathds{P}_{A\sim\chi}(\normx{f_n-\hat{f}}_\infty \geq \frac{2^\frac{i-1}{2}+2}{\sqrt{l}})\\
    &\leq  \sum_{i=1}^{2\log l}4e^{-\frac{1}{2}l(\frac{2^\frac{i-1}{2}-2}{\sqrt{l}})^2}\\
    &\leq  \sum_{i=1}^{2\log l}4e^{-\frac{1}{2}(2^\frac{i-1}{2}-2)^2}\\
    &\leq 4e^2 =O(1)
\end{align*}

Thus, the expected time searching each node to find the correct child is $O(T_k)$, and in total, the total expected time to traverse the tree for each insertion is $O(T_k \log\log k)$, since throughout, the height of the tree will be at most $\log\log k +1$ THIS IS NOT CORRECT FOR THE REBUILDING APPROACH. Furthermore, the cost of inserting a child into a leaf is at most $O(\log(C^2))$, which is $O(1)$. Thus, it remains to analyze the total cost of rebuilds.

Let $T(k)$ be the total number of operations performed for $k$ insertions. Let $B(k)$ be the total number of operations performed in the last rebuild of a tree at its root. That is, if the tree was rebuilt at $k$-th insertion and $\frac{k}{2}$-th insertion, $B(k)$ is the cost of operations between $\frac{k}{2}$-th and $k$-th. Thus, we have that $T(k)=B(k)+B(\frac{k}{2}+B(\frac{k}{4})+...)$. Since $B(k)$ is at least linear, we have that $\frac{1}{2}B(k)\geq B(\frac{k}{2})$, so that  $\sum_iB(\frac{k}{2^i})\leq\sum_i\frac{k}{2^i}B(k)\leq B(k)$ so that $T(k)=O(B(k))$.

Now, the root node has $\sqrt{k}$ children, and assume $k_i$ o[f the insertions were performed on the $i$-th child. Assume building a model over a sorted array of size $k$ takes $O(k)$, we have $B(k)=O(k)+\sum_i^{\sqrt{k}}T(\sqrt{k}, k_i)$. Similarly, $T(\sqrt{k}, k_i)=O(B(k_i+\sqrt{k}))=O(k_i+\sqrt{k}+\sum_j^{\sqrt{k_i+\sqrt{k}}}T(\sqrt{k_i+\sqrt{k}}, k_j))$


At any level $i$, $k$ insertions are collectively performed in all the nodes. Assume $k_j$ insertions are performed in the $j$-th node, so that 
\fi


==> proof_ce_two_d.tex <==
UNSURE IF THIS IS CORRECT
\subsubsection{Two Dimensions}

\begin{algorithm}[t]
\begin{algorithmic}[1]
\Require New element to be inserted in tree rooted at $N$
\Ensure Balanced data structure
\Procedure{Build}{$D$, $\epsilon$, $\psi$}
    \State $N\leftarrow $ new node
    \State $N.\hat{f}\leftarrow \textsc{BUILD\_Modle}(D)$
    \If {not $\textsc{IsVaid}(N.\hat{f})$}
        \State \Return $N$
    \EndIf
    \State $n\leftarrow |D|$
    \State $min\_est\leftarrow \sqrt{|D|}$
    \If {$n\leq\epsilon\psi$}
        \State \Return $N$
    \EndIf
    \State $Children\_max\_q\_ans\leftarrow \sqrt{n}(\frac{\sqrt{2\pi}}{\epsilon}+\log(\frac{4\sqrt{n}}{\psi\epsilon_r}))$
    \State $A\leftarrow argsort(D[:, 0])$
    %\State $D\leftarrow $ reordered $D$ according to $A$
    \State $D_w\leftarrow$ the first $Children\_max\_q\_ans$ of $D$
    \State $D_c\leftarrow D_w$
    \For {$i$ in  $Children\_max\_q\_ans$ to $n$}
        %\State $D_c\leftarrow D[i\sqrt{n}:(i+1)\sqrt{n}]$
%        \For {$p$ in $D_c$}    
        \State $p\leftarrow D[A[i]]$
        \If {$f(p)> Children\_max\_q\_ans$}
            \State continue
        \EndIf
        \State $D_c.append(p)$
        \State $D_w.append(p)$
        \State $p_max\leftarrow$ the point in $D_w$ with the largest $y$ coordinate
        \State Remove $p_max$ from $D_w$
        \If{$i mod Children\_max\_q\_ans==0$}
            \State $N.chilredn\_locs.append(p_max[1])$
            \State $N.chilredn.append(BUID(D_c))$
            \State $D_c\leftarrow D_w$    
        \EndIf
        \State $N.chilredn.BUID(D_c)$
    \EndFor
    \State $N.children.append(\textsc{BUILD}(D_c, \epsilon, \psi))$
    \State \Return $N$

\EndProcedure
\Procedure{Query}{$N$, $q$}
    \If {$N$ has no children}
        \State \Return $N.\hat{f}(q)$
    \EndIf
    \If {$N.\hat{f}(q)\geq \sqrt{n}(\frac{\sqrt{2\pi}}{\epsilon}+\log(\frac{4\sqrt{n}}{\psi\epsilon_r}))$}
        \State \Return $N.\hat{f}(q)$
    \EndIf
    \State $i\leftarrow binary\_search(N.chilredn\_locs, q[1])$
    \State \Return $\textsc{Query}(N.children[i], q)$
\EndProcedure
\caption{2-d one-sided card est}\label{alg:2d_card_est}
\end{algorithmic}
\end{algorithm}

First, assume that the model at some level is used to answer the queries. Thus, we have that either the model is invalid, or $\frac{\sqrt{n}}{\psi}\leq \epsilon_r$ or $\hat{f}(q)\geq \phi \sqrt{n}$.  

Note that if the model is invalid, the total error is at most $\frac{n}{\epsilon}$. $R_I$ be a random variable 0 if the model is valid and $\frac{n}{\epsilon}$, and let $R_V$ be equal to the relative error of using the model to answer queries when the model is valid and zero otherwise. Furthermore, let $R$ be the error of query answering. We have $E[R]=E[R_I+R_V]$. Note that $E[R_I]\leq\frac{n}{\psi}2e^{2(c-\phi)^2}=\epsilon_r$. THIS NEEDS MORE WORK, MAYBE THE IID THING


First, consider the case $\frac{\sqrt{n}}{\psi}\leq \epsilon_r$. PROVE IID Recall that we have 

\begin{align*}
    \mathds{P}(|\hat{f}(q)-f(q)|\leq \sqrt{n}\epsilon)\geq 1-2e^{-2\epsilon^2}
\end{align*}

%First, note that if $\frac{\sqrt{n}}{\psi}\leq \epsilon_r$, we have 
so
 
\begin{align*}
    \mathds{P}(\frac{|\hat{f}(q)-f(q)|}{\psi}\geq \frac{\epsilon\sqrt{n}}{\psi})\leq 2e^{-2(\epsilon^2)}
\end{align*}

and therefore

\begin{align*}
    \mathds{P}(\frac{|\hat{f}(q)-f(q)|}{\psi}\geq \epsilon \epsilon_r)\leq 2e^{-2(\epsilon^2)}
\end{align*}

which means

\begin{align*}
    \mathds{P}(\frac{|\hat{f}(q)-f(q)|}{\psi}\geq \epsilon )\leq 2e^{-2(\frac{\epsilon}{\epsilon_r})^2}
\end{align*}

Thus, in this case, $\mathds{E}(\frac{|\hat{f}(q)-f(q)|}{\max\{\psi, f(q)\}})\leq \frac{|\hat{f}(q)-f(q)|}{\psi}=\int_0^\infty\mathds{P}(\frac{|\hat{f}(q)-f(q)|}{\psi}\geq \epsilon )\leq \int_0^\infty2e^{-2(\frac{\epsilon}{\epsilon_r})^2}\leq \sqrt{\frac{\pi}{2}}\epsilon_r$  NEEDS SOME FIXING

Now assume $\frac{\sqrt{n}}{\psi}> \epsilon_r$ but $\hat{f}(q)\geq \phi \sqrt{n}$. Note that $|\hat{f}(q)-f(q)|\leq \sqrt{n}\epsilon$ implies $f(q)\geq \hat{f}-\sqrt{n}\epsilon$, so that for queries where $\hat{f}(q)\geq \phi \sqrt{n}$, we have whenever $|\hat{f}(q)-f(q)|\leq \sqrt{n}\epsilon$ we also have $\frac{|\hat{f}(q)-f(q)|}{\max\{f(q), \psi\}}\leq\min\{\frac{\epsilon}{\phi-\epsilon}, \frac{\epsilon\sqrt{n}}{\psi}\}$. 


Thus, for $0\leq\epsilon<\phi-\frac{\psi}{\sqrt{n}}$, we have 

\begin{align*}
    \mathds{P}(\frac{|\hat{f}(q)-f(q)|}{\max\{\psi, f(q)\}}\leq \frac{\epsilon}{\phi-\epsilon})\geq 1-2e^{-2\epsilon^2}.
\end{align*}

and therefore, for $0\leq \epsilon<\frac{\phi\sqrt{n}}{\psi}-1$
\begin{align*}
    \mathds{P}(\frac{|\hat{f}(q)-f(q)|}{\max\{\psi, f(q)\}}\geq \epsilon)\leq 2e^{-2(\frac{\phi\epsilon}{1+\epsilon}
    )^2}.
\end{align*}

and for $\epsilon\geq \phi-\frac{\psi}{\sqrt{n}}$

\begin{align*}
    \mathds{P}(\frac{|\hat{f}(q)-f(q)|}{\max\{\psi, f(q)\}}\leq \frac{\epsilon\sqrt{n}}{\psi})\geq 1-2e^{-2\epsilon^2}.
\end{align*}

Rearranging, we have for $\epsilon\geq\frac{\phi\sqrt{n}}{\psi}-1$

\begin{align*}
    \mathds{P}(\frac{|\hat{f}(q)-f(q)|}{\max\{\psi, f(q)\}}\geq \epsilon)\leq 2e^{-2(\frac{\epsilon\psi}{\sqrt{n}})^2}.
\end{align*}

Now, we have

\begin{align*}
    E[\frac{|\hat{f}(q)-f(q)|}{\max\{\psi, f(q)\}}]=\int_0^\infty\mathds{P}(\frac{|\hat{f}(q)-f(q)|}{\max\{\psi, f(q)\}}\geq \epsilon)\\
    \leq \int_0^{\frac{\phi\sqrt{n}}{\psi}-1}2e^{-2(\frac{\phi\epsilon}{1+\epsilon})^2}+\int_{\frac{\phi\sqrt{n}}{\psi}-1}^\infty 2e^{-2(\frac{\epsilon\psi}{\sqrt{n}})^2}
\end{align*}

We have that $\phi\frac{\sqrt{n}}{\psi}-1\geq \phi\epsilon_r-1=1$. Thus, consider the second term. We have 

\begin{align*}
    \int_{\frac{\phi\sqrt{n}}{\psi}-1}^\infty 2e^{-2(\frac{\epsilon\psi}{\sqrt{n}})^2}&=\frac{2\sqrt{n}}{\sqrt{2}\psi}\int_{\sqrt{2}(\phi-\frac{\psi}{\sqrt{n}})}^\infty e^{-t^2}dt\\
    &=\frac{\sqrt{0.5\pi}\sqrt{n}}{{\psi}}\text{erfc}(\sqrt{2}(\phi-\frac{\psi}{\sqrt{n}}))\\
    &\leq \frac{\sqrt{n}}{{\psi}}\frac{e^{-2(\phi-\frac{\psi}{\sqrt{n}})^2}}{4(\phi-\frac{\psi}{\sqrt{n}})}
\end{align*}

Now set $\phi\geq \sqrt{\frac{1}{2}\log(\frac{e\sqrt{n}}{\epsilon_r\psi})}+\frac{\psi}{\sqrt{n}}$. We have

\begin{align*}
    \frac{\sqrt{n}}{{\psi}}\frac{e^{-2(\sqrt{\frac{1}{2}\log(\frac{e\sqrt{n}}{\epsilon_r\psi})})^2}}{4(\sqrt{\frac{1}{2}\log(\frac{e\sqrt{n}}{\epsilon_r\psi})})}=\frac{\epsilon_r}{4e(\sqrt{\frac{1}{2}\log(\frac{e\sqrt{n}}{\epsilon_r\psi})})}\leq \epsilon_r
\end{align*}

where the last inequality follows because $\frac{\sqrt{n}}{\psi}\geq \epsilon_r$, so that $\frac{\sqrt{n}}{\psi}\geq \epsilon_r$.

Now consider the first term. We have, when $\frac{\phi\sqrt{n}}{\psi}-1\leq 1$

\begin{align*}
    \int_0^{\frac{\phi\sqrt{n}}{\psi}-1}2e^{-2(\frac{\phi\epsilon}{1+\epsilon})^2} \leq \int_0^{1}2e^{-2(\frac{\phi\epsilon}{1+\epsilon})^2}
    =\frac{\sqrt{2\pi}}{\phi}\text{erf}(\frac{\phi}{\sqrt{2}})
\end{align*}

Otherwise, 

\begin{align*}
    \int_0^{\frac{\phi\sqrt{n}}{\psi}-1}2e^{-2(\frac{\phi\epsilon}{1+\epsilon})^2} \leq \int_0^{1}2e^{-2(\frac{\phi\epsilon}{1+\epsilon})^2}+\sum_{i=1}^{\frac{\phi\sqrt{n}}{\psi}}2e^{-2(\phi\frac{i}{1+i})^2}\\
    \leq \frac{\sqrt{2\pi}}{\phi}+\frac{\phi\sqrt{n}}{\psi}e^{-\frac{\phi}{2}^2}\\
    \leq \frac{\sqrt{2\pi}}{\phi}+\frac{4\sqrt{n}}{\psi}e^{-\phi}
\end{align*}

Bounding the first term, we have $\phi\geq\frac{\sqrt{2\pi}}{\epsilon}$ and bounding the second term, we have $\phi\geq\log(\frac{4\sqrt{n}}{\psi\epsilon_r})$. Thus, setting $\phi=\frac{\sqrt{2\pi}}{\epsilon}+\log(\frac{4\sqrt{n}}{\psi\epsilon_r})$ bounds the total error by $(2+\frac{\pi}{2})\epsilon_r$.


==> sorting_backup.tex <==

Note that

\begin{align*}
\normx{\hat{f}-f'_n}_\infty&\leq \normx{\hat{f}-f_{\sqrt{n}}}_\infty+\normx{f_{\sqrt{n}}-f_\chi}+\normx{f_\chi-f'_{n}}_\infty
\end{align*}

We have that $\mathds{P}(\normx{f_{\sqrt{n}}-f_\chi}\geq \epsilon_2)\leq 2e^{2\sqrt{n}\epsilon_2^2}$ and $\mathds{P}(\normx{f_n-f_\chi}\geq \epsilon_3)\leq 2e^{2n\epsilon_3^2}$ so that 

\begin{align*}
\mathds{P}(\normx{\hat{f}-f_{\sqrt{n}}}_{\infty}\geq \epsilon_1 \text{\;or\;} \normx{f_{\sqrt{n}}-f_\chi}\geq \epsilon_2 \text{\;or\;} \normx{f_n-f_\chi}\geq \epsilon_3)\\\leq 2e^{-2\sqrt{n}\epsilon_2^2}+2e^{-2n\epsilon_3^2}+2e^{2\sqrt{n}\epsilon_1^2}    
\end{align*}

Set $\epsilon_1=\epsilon_2=\sqrt{\frac{\log\log n}{\sqrt{n}}}$ and $\epsilon_3=\sqrt{\frac{\log\log n}{n}}$, we have
    
\begin{align*}
\mathds{P}(\normx{\hat{f}-f_{\sqrt{n}}}_{\infty}\geq \epsilon_1 \text{\;or\;} \normx{f_{\sqrt{n}}-f_\chi}\geq \epsilon_2 \text{\;or\;} \normx{f_n-f_\chi}\geq \epsilon_3)\\
\leq 2e^{-\log\log n}+2e^{-\log\log n}+2e^{-\log\log n}\\
=\frac{6}{\log n}
\end{align*}

Thus, 

$$
\mathds{P}(\normx{\hat{f}-f'_n}\geq \epsilon_1+\epsilon_2+\epsilon_3)\leq \frac{6}{\log n}
$$

and thus

$$
\mathds{P}(\normx{\hat{f}-f'_n}_\infty\geq 3n^{-\frac{1}{4}}\sqrt{\log\log n})\leq \frac{6}{\log n}
$$

Now consider the $i$-th bucket. The elements, $x$, assigned to it must have $\frac{i}{k}\leq \hat{f}(x)<\frac{i+1}{k}$. Combining this with the above, we have that whenever $\normx{\hat{f}-f'_n}_\infty\geq 3n^{-\frac{1}{4}}\sqrt{\log\log n}$ holds, for the elements, $x$, in the $i$-th bucket, we must have $f'_n(x)\geq \frac{i}{k}-3n^{-\frac{1}{4}}\sqrt{\log\log n}$ and that $f'_n(x)\leq \frac{i+1}{k}+3n^{-\frac{1}{4}}\sqrt{\log\log n}$. Therefore, we must have $nf'_n(x)\in [\frac{in}{k}-3n^{\frac{3}{4}}\sqrt{\log\log n}, \frac{(i+1)n}{k}+3n^{\frac{3}{4}}\sqrt{\log\log n}]$. There are at most $\frac{n}{k}+6n^{\frac{3}{4}}\sqrt{\log\log n}$ elements in this set. Setting $k=\frac{n^{\frac{1}{4}}}{\sqrt{\log\log n}}$, we have that whenever $\normx{\hat{f}-f'_n}_\infty\geq 3n^{-\frac{1}{4}}\sqrt{\log\log n}$ holds, all buckets will have at most $7n^{\frac{3}{4}}\sqrt{\log\log n}$ elements. Thus, the probability that a bucket will have more than $7n^{\frac{3}{4}}\sqrt{\log\log n}$ elements is at most $\frac{6}{\log n}$

Furthermore, the largest element in the $i$-th bucket or before will have $nf'_n(x)< (i+4)n^{\frac{3}{4}}\sqrt{\log\log n}$ and the smallest element in the $i+7$-th bucket or after will have $nf'_n(x)\geq (i+4)n^{\frac{3}{4}}\sqrt{\log\log n}$, so that the content of buckets up to $i$ are less than the content of the buckets from $i+7$ onwards.

Thus, if all the buckets are sorted, then the algorithm takes at most $\sum_{i=1}^k(\sum_{j=0}^7|B_{i-j}|$ number of operations to sort the merge the sorted array, which is $O(n)$. 

\if 
Now use $n\hat{f}$ to group the elements into $k$ groups, where an element is assigned to the group $\floorx{k\hat{f}}$. Observe that for an element to be assigned to the $i$-th group, we need to have 



insert the elements into the array, and group every $3n^{\frac{3}{4}}\sqrt{\log\log n}$ elements together. Let $k = 3n^{\frac{3}{4}}\sqrt{\log\log n}$,  Let $\bar{N}_{k, i}$ be the size of the number of points in the $i$-th group. Also consider grouping the slots of every $3$ consecutive groups, so that $N_{3k, i}=\sum_{j=0}^{3k}N_{i+j}$. Note that $\bar{N}_{k, i}\leq N_{3k, i-1} $. 
\fi

Let $I_M$ denote the event of doing a merge sort. We have

\begin{align*}
    E[T(A)]&=n+E[I_MT_M+(1-I_M)\sum_{i=1}^{\frac{n}{k}}T(A_i)]\\
    &\leq n+\frac{6}{\log n}n\log n+E[\sum_{i=1}^{\frac{n}{k}}T(A_i)]\\
    &=O(n)+E[\sum_{i=1}^{\frac{n}{k}}T(A_i)]\\
    &=O(n\log\log n)
\end{align*}

THIS PROBABLY NEEDS MORE DISCUSSION TWO, NOT OBVIOUS WHY RECURSION APPLIES



\subsubsection{Using data distribution}

\begin{algorithm}[t]
\begin{algorithmic}[1]
\Require An unsorted array $A$ of size $n$
\Ensure A sorted array
\Procedure{Sort}{$A$}
    \If{$n\leq 10$}
        \Return{$MergeSort(A)$}
    \EndIf
    \State $A'\leftarrow$ array of size $n$, initialized with nulls
    \For{$i\leftarrow 1$ to $n$}
        \State $i'\leftarrow \ceilx{nf_\chi(A[i])}$
        \If{$A'[i']\neq \text{NULL}$}\label{alg:sort_dist:map}
            \State $A[i].\text{next}\leftarrow A[i].\text{next}$
            \State $A'[i'].\text{next}\leftarrow A[i]$
        \Else
            \State $A'[i']\leftarrow A[i]$
        \EndIf
    \EndFor
    \State $i\leftarrow 0$
    \For{$j\leftarrow 0$ to $n$}
        \If{$A'[j]=\text{NULL}$}
            \State \textbf{continue}
        \EndIf
        \State $S = MergeSort(A'[j])$
        \For{$k\leftarrow 0$ to $|S|$}
            \State $A'[i]=S[k]$
            \State $i++$            
        \EndFor
    \EndFor
    \Return{$A'$}
\EndProcedure
\caption{Sorting}\label{alg:dist_sort}
\end{algorithmic}
\end{algorithm}

Alg.~\ref{alg:dist_sort} shows how to sort an array given the cdf of the distribution $\chi$ the data was sampled from.

\textbf{Correctness}
The algorithm first iterates over the array and inserts the elements into a new array, where $A[i]$ is inserted at $A'[\ceilx{nf_\chi(A[i])}]$. $f_\chi$ is an increasing function, so that $\ceilx{nf_\chi(A[i])}\leq \ceilx{nf_\chi(A[j])}$ iff  $A[i]\leq A[j]$, so that $A'$ will contain the elements of $A$ in the correct order. However, multiple elements may be mapped to, $A'[i]$, for any index $i$, which are therefore stored in a linked list from $A'[i]$.

The algorithm then scans $A'$, for any location $A'[j]$ where multiple elements are mapped (i.e., there is a linked list), the linked list is first recursively sorted and the sorted list is then inserted to the first empty location available in $A'$. Thus, the final returned  $A'$ will be sorted.

\textbf{Running time}
Let ${T}(A)$ be the number of operations the algorithm performs on an array $A$, and let $\mathcal{T}(n)=\mathds{E}_{A\sim\chi^n}[{T}(A)]$ be the expected run time of the algorithm on an input of size $n$. 

Note that, in line \ref{alg:sort_dist:map}, an element, $A[i]$ is mapped to a location $i'$ if c.d.f of  $A[i]$ is between $\frac{i'-1}{n}< f_\chi(A[i])\leq \frac{i'}{n}$. Thus, probability that $A[i]$ is mapped to location $i'$ is $\frac{1}{n}$. XXX reference that CDF of any random variable is uniformly distributed. Let $N_j=|A'[j]|$ be the number of elements mapped to the $j$-th location. For any $i$, we have that $$\mathds{P}_{A\sim\chi^n}(N_j=i)=\mathds{C}(n, i)(\frac{1}{n})^i(1-\frac{1}{n})^{n-i}$$, since probability that any sample falls in $(\frac{j-1}{n}, \frac{j}{n}]$ is $\frac{1}{n}$, and we are taking $n$ independent samples. 

Thus, we have that $T(A)=cn+\sum_{j=1}^n{N_j\log(N_j)}$. So that 

\begin{align*}
\mathds{E}_{A\sim\chi^n}[T(A)]&=cn+\sum_{j=1}^n{\mathds{E}_{A\sim\chi^n}[N_j\log(N_j)]}\\
&=cn+\sum_{j=1}^n\sum_{i=1}^{n}\mathds{P}_{A\sim\chi^n}(N_j=i)[i\log(i)]\\
&=cn+\sum_{j=1}^n\sum_{i=1}^{n}\mathds{C}(n, i)(\frac{1}{n})^i(1-\frac{1}{n})^{n-i}i\log i\\
&\leq cn+\sum_{i=1}^{n}n(\frac{en}{i})^i(\frac{1}{n})^ii^2\\
&= cn+e^2\sum_{i=1}^{n}n(\frac{e}{i})^{i-2}\\
&= cn+e^2(\sum_{i=1}^{6}n(\frac{e}{i})^{i-2} +\sum_{i=6}^{n}n(\frac{e}{i})^{i-2})\\
&\leq cn+e^2(n(6e^4)+\sum_{i=6}^{n}n(\frac{e}{i})^{i-2}) \\
&\leq cn+e^2(n(6e^4)+\sum_{i=6}^{n}n(\frac{1}{2})^{i-2}) \\
&\leq cn+e^2(n(6e^4)+n\sum_{i=4}^{\infty}(\frac{1}{2})^{i}) \\
&\leq cn+e^2(n(6e^4)+2n) \\
&= O(n)
\end{align*}

\if 0
We have that $T(A)=cn+\sum_j{T(A'[j])}$. So that $\mathds{E}_{A\sim\chi^n}[T(A)]=cn+\sum_j{\mathds{E}_{A\sim\chi^n}[T(A'[j])]}$

Note that $\mathds{E}_{A\sim\chi^n}[T(A'[j])]$ is the expected time of sorting elements from $A$ whose cdf is between $\frac{j-1}{n}< f_\chi(A[i])\leq \frac{j}{n}$
\fi

Alternatively, consider grouping every $k$ array index and sorting every $k$ combined. Thus, we have

\begin{align*}
\mathds{E}_{A\sim\chi^n}[T(A)]&=cn+\sum_{j=1}^{n/k}{\mathds{E}_{A
\sim\chi^n}[N_j\log(N_j)]}\\
&=cn+\sum_{j=1}^{n/k}\sum_{i=1}^{n}\mathds{P}_{A\sim\chi^n}(N_j=i)[i\log(i)]\\
&=cn+\sum_{j=1}^{n/k}\sum_{i=1}^{n}\mathds{C}(n, i)(\frac{k}{n})^i(1-\frac{k}{n})^{n-i}i\log i\\
\end{align*}

For $k=o(n)$ we have 

\begin{align*}
&=cn+\frac{n}{k}\sum_{i=1}^{n}\mathds{C}(n, i)(\frac{k}{n})^i(1-\frac{k}{n})^{n-i}i\log i\\    
&=cn+\frac{n}{k}(\sum_{i=1}^{4ek}\mathds{C}(n, i)(\frac{k}{n})^i(1-\frac{k}{n})^{n-i}i\log i+\sum_{i=4ek}^{n}\mathds{C}(n, i)(\frac{k}{n})^i(1-\frac{k}{n})^{n-i}i\log i)\\    
&\leq cn+\frac{n}{k}(\sum_{i=1}^{4ek}\mathds{C}(n, i)(\frac{k}{n})^i(1-\frac{k}{n})^{n-i}i\log i+\sum_{i=4ek}^{n}\frac{1}{\sqrt{i}}(\frac{en}{i})^i(\frac{k}{n})^i(1-\frac{k}{n})^{n-i}i\log i)\\
&= cn+\frac{n}{k}(\sum_{i=1}^{4ek}\mathds{C}(n, i)(\frac{k}{n})^i(1-\frac{k}{n})^{n-i}i\log i+\sum_{i=4ek}^{n}(\frac{ekn}{i(n-k)})^i(1-\frac{k}{n})^{n}\sqrt{i}\log i)\\
&\leq cn+\frac{n}{k}(\sum_{i=1}^{4ek}\mathds{C}(n, i)(\frac{k}{n})^i(1-\frac{k}{n})^{n-i}i\log i+\sum_{i=4ek}^{n}(\frac{2ek}{i})^i(1-\frac{k}{n})^{n}\sqrt{i}\log i)\\
&\leq cn+\frac{n}{k}(\sum_{i=1}^{4ek}\mathds{C}(n, i)(\frac{k}{n})^i(1-\frac{k}{n})^{n-i}i\log i+\sum_{i=4ek}^{n}(\frac{1}{2})^ii)\\
&\leq cn+\frac{n}{k}(\sum_{i=1}^{4ek}\mathds{C}(n, i)(\frac{k}{n})^i(1-\frac{k}{n})^{n-i}i\log i+2)\\
&\leq cn+\frac{n\log(4ek)}{k}(\sum_{i=1}^{4ek}\mathds{C}(n, i)(\frac{k}{n})^i(1-\frac{k}{n})^{n-i}i+2)\\
&\leq cn+\frac{n\log(4ek)}{k}(n\times\frac{k}{n}+2)\\
&=O(n\log k)
\end{align*}


Now assume we have a function approximator with error $\normx{\hat{f}-f_\chi}_\infty\leq \epsilon$ that takes $B_{n, \epsilon}$ to build, $T_{n, \epsilon}$ to evaluate, and space $S_{n, \epsilon}$. 

We have that $\normx{\hat{f}-nf_\chi}_\infty\leq \epsilon$. Thus, if, for any $i$,  $nf_\chi(A[i])=j$, $\hat{f}\in \{j-\floorx{\epsilon}, ..., j+\ceilx{\epsilon}\}$. %Let $\hat{N}_j$ be the number of elements mapped to $A'[i]$ if we use $\hat{f}$ instead of $f_\chi$. Note that $\hat{N}_j\leq \sum_{j-n\epsilon}^{j+n\epsilon}N_j$. 

%We will group that items into groups of $\ceilx{n\epsilon}$, and call mergesort on every $\ceilx{n\epsilon}$ group separately. Thus, we have. Let $\bar{N}_k$ be the size of the $k$-th such group, out of a total of $K=\frac{n}{\ceilx{n\epsilon}}$ groups. 

Let $k=\epsilon$. Let $\bar{N}_{k, i}$ be the size of the slots grouped into groups of $k$. Consider the groups of every $3$ slots, so that $N_{3k, i}=\sum_{j=0}^{3k}N_{i+j}$. Note that $\bar{N}_{k, i}\leq N_{3k, i-1} $. 


We have 

\begin{align*}
\mathds{E}_{A\sim\chi^n}[\hat{T}(A)]&=\mathds{E}_{A\sim\chi^n}[B_{n, \epsilon}+nT_{n, \epsilon}]+\sum_{j=1}^{\frac{n}{k}}{\mathds{E}_{A\sim\chi^n}[\bar{N}_{k, j}\log(\bar{N}_{k, j})]}\\
&\leq \mathds{E}_{A\sim\chi^n}[B_{n, \epsilon}+nT_{n, \epsilon}]+\sum_{j=1}^{\frac{n}{k}}{\mathds{E}_{A\sim\chi^n}[N_{3k, j-1}\log(N_{3k, j-1})]}\\
&\leq \mathds{E}_{A\sim\chi^n}[B_{n, \epsilon}+nT_{n, \epsilon}]+\frac{n}{k}{3k\log(3k)}\\
&=O(\mathds{E}_{A\sim\chi^n}[B_{n, \epsilon}+nT_{n, \epsilon}]+n\log k)\\
&=O(nT_{\epsilon}+n\log \epsilon)
\end{align*}
